A Hierarchical Assessment of Adversarial Severity

Adversarial Robustness is a growing field that evidences the brittleness of neural networks. Although the literature on adversarial robustness is vast, a dimension is missing in these studies: assessing how severe the mistakes are. We call this notion "Adversarial Severity" since it quantifies the downstream impact of adversarial corruptions by computing the semantic error between the misclassification and the proper label. We propose to study the effects of adversarial noise by measuring the Robustness and Severity into a large-scale dataset: iNaturalist-H. Our contributions are: (i) we introduce novel Hierarchical Attacks that harness the rich structured space of labels to create adversarial examples. (ii) These attacks allow us to benchmark the Adversarial Robustness and Severity of classification models. (iii) We enhance the traditional adversarial training with a simple yet effective Hierarchical Curriculum Training to learn these nodes gradually within the hierarchical tree. We perform extensive experiments showing that hierarchical defenses allow deep models to boost the adversarial Robustness by 1.85% and reduce the severity of all attacks by 0.17, on average.

==> sections/01old_introduction.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[width=0.95\textwidth]{images/h-attacks.png}
    \caption{\textbf{Hierarchical Attacks.} In contrast to standard adversarial attacks in (a), we generate adversarial perturbations by considering the hierarchical distance between labels. Given a level $l=2$, in (b) LHA generate the examples by taking into account only the classes with a hierarchical distance lower or equal than $l$. Similarly, (c) GHA uses those that are higher or equal than $l$. Lastly, (d) NHA considers the father nodes with a height level of $l$ as the classification nodes and generate the adversaries in order perturb this classification.} 
    \label{fig:h-attacks}
\end{figure*}

\section{Introduction}

%Deep Learning (DL) has proven effective to tackle multiple tasks, achieving unprecedented performances. The literature shows that deep learning techniques~\cite{krizhevsky2012imagenet, vgg15, resnet16, googlenet15, unet15, maskrcnn17, Kirillov_2019_CVPR} are the predominant models to engage a broad span of challenging tasks, such as Classification \cite{ILSVRC15, inat19}, Segmentation \cite{pascal15, amfm_pami2011}, Detection \cite{Geiger2012CVPR}, Instance Segmentation \cite{coco14} and Panoptic Segmentation \cite{Kirillov_2019_CVPR}. Although DL models are outstanding tools, they have been shown to be remarkably brittle against malicious noises, known as adversarial attacks. In particular, studies have shown that these attacks have the capacity of dropping the performance of DL models to nearly 0\% \cite{madry2017} while being invisible to the human eye. These attacks exploit all image regions to fool a network in order to move its prediction across decision boundaries.

Research on adversarial robustness is growing at an accelerated pace. Since the introduction of Fast Sign Gradient Method (FSGM) \cite{goodfellow2015explaining}, numerous works have emerged in order to attack \cite{croce2020reliable, square2020, croce2020minimally} and defend \cite{madry2017, zhang2019theoretically} models. Nonetheless, prior works focus exclusively on how adversarial attacks flip the network's decision, without considering the severity of the error induced by the attack. Namely, there is no quantification of the semantic error induced by an adversarial perturbation, as modeled by the hierarchical distance within a set of labels governed by a tree. We call this notion \textit{Adversarial Severity}.

Widely-known adversarial attacks such as FSGM \cite{goodfellow2015explaining}, Projected Gradient Descent (PGD) \cite{madry2017} or AutoAttack (AA) \cite{croce2020reliable}, share a common objective: they aim solely at harming accuracy. While this spirit follows a strong focus on top-1 accuracy, we note that attacks developed with such focus do not exploit the class hierarchy. Thus, we introduce hierarchy-aware attacks. In particular, we propose a new suite of hierarchical attacks that target both the accuracy and the hierarchical error. Unlike these attacks, the suite is composed of three attacks that harness the rich semantic structure of the label space in order to impact the model in multiple manners. Figure \ref{fig:h-attacks} shows an overview of how \textit{(a)} Standard Untargeted methods ignores the rich semantic structure of the label space and how \textit{(b-d)} our attacks, dubbed \textit{Lower Hierarchical Attack} (LHA), \textit{Greater Hierarchical Attack} (GHA) and \textit{Node-based Hierarchical attack} (NHA), enjoy from this information to measure the robustness, that create adversaries in order to fool the network based on a hierarchical distance criterion: \textit{(i)} LHA creates distortions with low hierarchical distances, \textit{(ii)} GHA attacks the target image by pretending to fool the target network with highly dissimilar semantics, and \textit{(iii)} NHA crafts adversarial images in order to change the parent node.

To deploy machine learning algorithms in real-life scenarios, we require them to be protected against adversarial attacks capable of radically changing the model's output. That is, we require models that are robust against adversaries. In many real-life scenarios, such as Robot-Assisted Surgeries, some mistakes are not considered as severe as others. Take as an example a laparoscopy surgery. There are diverse moments when several tools are not used. Therefore, interchanging the labels of these unused implements is not as important as misclassifying any of those with the target in the surgery.% \juan{The point stated in this paragraph is very important. However, I think there may be a simpler example to illustrate this point.} \guillaume{We could talk about security cameras or self-driving cars}

Since the introduction of DL models, utilizing the hierarchical information as an additional source of information has been cast aside to some extent. Recently, Bertinetto \etal~\cite{bertinetto2020making} studied how modern progress in DL has come at no such improvements in terms of hierarchical error, despite providing large gains in classification accuracy. Our work follows a similar vein by exploiting adversarial attacks: no work has quantified the semantic errors in which networks incur when subjected to adversarial attacks. So, we provide a complete benchmark of the impact of adversarial attacks in hierarchical errors, and propose a technique to mitigate such errors.

%\guillaume{paragraph here for the benchmarking? or simply extend the last one... although I think it is just fine as it is}

% \begin{figure}[t]
%     \centering
%     %\fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
%     \includegraphics[width=\columnwidth]{images/pull fig.png}
%     \caption{\textbf{Adversarial Robustness and Severity assessment.} Our study reviews the effect of adversarial attacks by assessing both Robustness (a) and Severity (b). The newly introduced attacks harm both accuracy (higher is better) and the average mistake (lower is better). Simultaneously, our proposed curriculum boosts the accuracy and reduces the average mistake.}
%     \label{fig:pull_fig}
% \end{figure}



In this paper, we hypothesize that the inclusion of the hierarchy into the adversarial training enhances the robustness against adversarial attacks. Thus, our approach takes inspiration from curriculum-based human learning \cite{Bengio_Currulum_ICML09, jae11learning}. Intuitively, a student's learning journey starts from basic and coarse concepts and goes towards finer and specialized ones. This mechanism allows the student to easily learn finer concepts as the coarse notions may serve as a strong prior for them. While in many tasks is troublesome to define concepts as coarse/fine, we exploit the fact that these are easily defined when there is an underlying hierarchical structure encompassing the classes. Consequently, we incorporate a hierarchical curriculum training to gradually learn all nodes at every level in the class hierarchy. Our technique proves to be effective: our experiments show that the curriculum-enhanced training improves both robustness and diminishes the error severity of neural networks when under attack. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\guillaume{Above this will be the old introduction. I'll have it uncommented whenever we want to check some old things.}

\noindent\rule{8cm}{0.4pt}


==> sections/03old_method.tex <==
% \guillaume{CAMBIOS:}

% \begin{enumerate}
%     \item Ataques
%     \item Benchmark (pasar de métodos)
%     \item Curriculo
% \end{enumerate}

\section{Methods}
%We divide our methodology into four sections. First, we introduce notations. Second, we describe our new hierarchy-aware adversarial attacks. Then, we present the benchmark to assess the adversarial robustness and severity. Lastly, we present our novel training curriculum aimed at exploiting hierarchical information from the class tree to enhance adversarial robustness.

%\guillaume{in case of space, we can simply comment this.}

\subsection{Notation} \label{sec:notation}

A hierarchical tree with depth $L$ is a set of groups of nodes $\{Y_1, Y_2, ..., Y_L\}$ and their corresponding transition functions $C_{l, l'}$ between levels. Let $Y_l = \{1, 2, ..., n_l\}$ be the set of nodes at level $l$. A transition function $C_{l, l'}$ maps any label in $Y_l$ into a subset of nodes in $Y_{l'}$, representing the label's offspring when $l<l'$. Formally, $C_{l,l'}: Y_l \rightarrow \mathbb{P}(Y_{l'})$, where $\mathbb{P}(A)$ is the powerset of a set $A$. These transition operations have the following properties:

\begin{enumerate}
    \item $\bigcup_{i \in Y_l} C_{l,l'}(i) = Y_{l'}$
    \item $C_{l,l'}(i) \neq \varnothing$, $\forall i \in Y_l$
    \item $C_{l,l'}(i) \cap C_{l,l'}(j) = \varnothing$, $\forall i, j \in Y_l$, $i \neq j$ if $l \leq l'$.
\end{enumerate}

To measure distances within the topology of a tree, we use the hierarchical distance $d_H$. This metric is defined as the height of least common ancestor between nodes. So, we use $d_H$ to measure a semantic difference between an instance's prediction and the corresponding ground-truth. Throughout the rest of the manuscript, we refer as \textit{mistake} as the hierarchical distance between two nodes.

Let be a dataset with images and their corresponding hierarchical labels from the tree. Suppose the current task is to classify images from the dataset only with respect to the labels from $Y_l$. Let a neural network be a composition between a backbone $g_\Theta$ that extract features representation of images and a linear classifier $f_{W^l, b^l}$. $\Theta$ is the set of all parameters of $g$ and $W^l \in \mathbb{R}^{n_l \times m}$ and $b^l \in \mathbb{R}^{n_l}$ are the weights and biases of $f$, respectively. $m$ is the feature dimension of the representation vector. Define $W_i^l \in \mathbb{R}^{1 \times m}$ to be the $i$-th row of $W^l$ and $b_{i}^l \in \mathbb{R}$ to be the $i$-th component of the bias vector.

\subsection{Hierarchical Attacks}

In order to assess the severity of adversarial attacks, we propose novel hierarchy-aware adversaries that perturb images aiming at both the reducing standard accuracy and increasing the severity of hierarchical mistakes. Figure \ref{fig:h-attacks} provides a graphical illustration of our new attacks: \textit{Lower Hierarchical Attack}, \textit{Greater Hierarchical Attack} and \textit{Node-based Hierarchical Attack}. As we intend to increase hierarchical mistakes as well, all our attacks aim at extracting and harming the target image by exploiting the rich structure of the hierarchy.
 
\textbf{Lower and Greater Hierarchical Attacks at level $l$.} These attacks aim at perturbing the target image by creating distortions based on a criterion related to the hierarchical distance at level $l$. Both attacks operate on a similar way: to choose the target classes depending on the severity of the attack, given by $l$. Please refer to Figure \ref{fig:h-attacks}b and \ref{fig:h-attacks}c for an illustration of the intuition behind our proposed attacks.

On the one hand, the easier labels for the attack to target are those whose similarity within the tree is at most $l$ in the hierarchical distance. Accordingly, LHA creates the adversarial examples targeting classes whose distance to the original class is less than or equal to $l$. Thus, for an image $x$ and its leaf label $y$, LHA optimizes the loss (Equation \eqref{eq:LHA})
\begin{equation}\label{eq:LHA}
    \begin{split}
        L_{LHA @ l}(x, y)& = \\
        -\log &\frac{e^{W^L_y g_\Theta(x) + b^L_y}}{\sum_{j \in Y_L \text{ s.t. } d_H (y,j) \leq l} e^{W^L_j g_\Theta(x) + b^L_j}}.
    \end{split}
\end{equation}

On the other hand, GHA@$l$ aims at creating adversaries that induce large mistakes (\textit{i.e.} cause remarkable ``confuse'' of the network). Conversely to LHA, GHA uses information from the classes with a hierarchical distance \textit{greater} or equal to $l$. Thus, GHA maximizes the loss (Equation \eqref{eq:GHA})
\begin{equation}\label{eq:GHA}
    \begin{split}
        L_{GHA @ l}(x&, y) = \\
         -\log & \frac{e^{W^L_y g_\Theta(x) + b^L_y}}{\sum_{j \in \{k \in Y_L | d_H(y,k) \geq l \text{ or } k=y \} } e^{W^L_j g_\Theta(x) + b^L_j}}.
    \end{split}
\end{equation} % queda horrible si se separa la suma

To ease the understanding of these losses, we point out that the objective to minimize is similar for both attacks. On Figure \ref{fig:h-attacks}b and \ref{fig:h-attacks}c, in essence, both attacks harms the purple node -the label- by using as negative classes the red leaves.


\textbf{Node-based Hierarchical Attacks.} The NHA harms the nodes with a height of $l$. Figure \ref{fig:h-attacks}d exemplifies our proposed attack. The probability of classifying a target image $x$ as a node $y$ with height $l$ is equal to the sum of the probabilities of choosing any leaf class derived from $y$. Therefore,
\begin{equation}\label{eq:prob-of-node}
    P(c(x)=y \in Y_{L - l}) = \sum_{i \in C_{L-l,L}(y)} P(c(x) = i \in Y_L)
\end{equation}
where $c(x) = y$ is the action of classifying $x$ as $y$ and $P(c(x)=y \in Y_{L-l})$ is the probability of classifying $x$ as $y \in Y_{L-l}$. Note that the height of any $y \in Y_{L-l}$ is equal to $l$.
As is standard, all state-of-the-art models use a Softmax layer to compute the probability distribution of an input image by using the corresponding logits. Therefore, the probability of the neural network to classify $x$ as class $i$ is:
\begin{equation}
    P(c(x)=i \in Y_L| \Theta, W^L, b^L) = \frac{e^{W^L_i g_\Theta(x) + b^L_i}}{\sum_{j=1}^{n_L}e^{W^L_j g_\Theta(x) + b^L_j}}.
\end{equation}
Hence, following Equation \eqref{eq:prob-of-node}, the probability of classifying $x$ as $y \in Y_{L-l}$ is:
\begin{equation} \label{eq:prob-of-node-model}
    \begin{split}
        P(c(x)=y \in Y_{L-l} | \Theta,& W^L, b^L) = \\
        &\frac{\sum_{i \in C_{L-l,L}(y)}e^{W^L_i g_\Theta(x) + b^L_i}}{\sum_{j=1}^{n_L}e^{W^L_j g_\Theta(x) + b^L_j}}.
    \end{split}
\end{equation}

To extract adversaries based on Equation \eqref{eq:prob-of-node-model}, we compute the cross-entropy loss. %\juan{in the next sentence we mention that we ``alleviate this operation''. We must explain why this is important. Because of computational costs? Or because of numerical instability?}. 
To speed up this operation, we estimate the adversaries by attacking the cross-entropy on Equation \eqref{eq:NHA}. This function computes the loss over the maximum logits within nodes of interest:
\begin{equation} \label{eq:NHA}
    \Tilde{L}_{NHA@l}(x, y) = -\log \frac{e^{\Tilde{L}_{y}}}{\sum_{j=1}^{n_l} e^{\Tilde{L}_j}}
\end{equation}
where, $\Tilde{L}_y = \max_{i \in C_{L-l,L}(y)} W^L_i g_\Theta(x) + b^L_i$. We base our design on the mathematical principle that, if $L_y$ is the logit corresponding to node $y \in Y_{L-l}$, %. Although this logit is not computed directly by the model, 
with straightforward algebraic manipulation we can obtain that
\begin{equation} \label{eq:logit-node}
    L_y = \log \sum_{i \in C_{L-l,L}(y)}e^{W_i g_\Theta(x) + b_i}.
\end{equation}

% It is widely known that the $\max$ function has a variety of differentiable approximations. We recall one in particular: LogSumExp ($LSE$), shown in Equation \eqref{eq:lse}. By comparing Equation \eqref{eq:logit-node} and the $LSE$, we find that $L_y \approx \widetilde{L_y}$. As a results, we attack an approximation of the true cross-entropy function--Equation \eqref{eq:NHA}. Figure \ref{fig:h-attacks}d exemplifies our proposed attack.

% \begin{equation} \label{eq:lse}
% \begin{split}
%     LSE (x_1, ..., x_m) & = \log (e^{x_1} + ... + e^{x_m}) \\
%     & \approx \max(x_1, ..., x_m)
% \end{split}
% \end{equation}

It is widely known that the $\max$ function has a variety of differentiable approximations. We recall one in particular: $max (x_1, ..., x_m)
\approx \log (e^{x_1} + ... + e^{x_m})$. Thus, we find that $L_y \approx \Tilde{L}_y$. As a result, we attack an approximation of the true cross-entropy function--Equation \eqref{eq:NHA}. On Figure \ref{fig:h-attacks}d we exemplify the idea behind NHA. This attack extracts the maximum logit over the leaf offspring of each node at the target level. So, NHA harness these logits to create the adversary.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Benchmarking Adversarial Severity}

In order to conduct an assessment of both adversarial robustness and severity, we compute two metrics that reflect these concepts. First, we compute the standard \textit{Robust Accuracy}. This measurement quantifies the worst-case endurance of a defense against adversarial examples. However, this metric does not provide information about the semantic error in which the model incurred under the attack. Hence, we also compute the \textit{Average Mistake} \cite{bertinetto2020making}. By averaging the hierarchical distance $d_H$ of all misclassified instances. This metric quantifies the semantic difference between the prediction and the ground-truth label, thus, addressing the issue presented by only measuring accuracy.

Fundamentally, our attacks propose novel optimization objectives. In practice, for optimizing such objectives, we implement a PGD-based strategy. The standard PGD~\cite{madry2017} iteratively performs FSGM steps \cite{goodfellow2015explaining} to maximize the Cross-Entropy Loss $L$ between the prediction for an instance $x$ and its corresponding ground-truth label $y$ to find an adversarial example:
\begin{equation}\label{eq:pgd-attack}
    \begin{split}
    x_{t+1} = \prod_{B_{\ell_\infty}(x, \epsilon)} x_t + \alpha\:\text{sign}\left(\nabla_{x_t} (L(m(x_t), y))\right),
    \end{split}
\end{equation}
where $m(\cdot) = Softmax(f_{W^L, b^L}(g_\Theta(\cdot)))$, and the initial point $x_0$ is perturbed with noise, namely $x_0 = x + u$, with $u$ being sampled from the uniform random distribution $\mathcal{U}[-\epsilon, \epsilon]$, $\alpha$ is the step per iteration and $\prod_{A}$ is the projection function over the set $A$. The set $B_{\ell_\infty}(x, \epsilon)$ is the intersection of the $\epsilon$-ball with the $\ell_\infty$ norm around $x$ and the set $[0,1]^{size(x)}$. We refer to an $n$-step PGD attack as PGD\textbf{$n$}. Using PGD-optimization for our attacks amounts to replacing the Loss $L$ in Equation \eqref{eq:pgd-attack} with each of the losses in Equations \eqref{eq:LHA}, \eqref{eq:GHA} and \eqref{eq:NHA}. Analogously, we refer to the $n$-step versions of these attacks as LHA\textbf{$n$}@$l$, GHA\textbf{$n$}@$l$ and NHA\textbf{$n$}@$l$. For all our evaluation experiments, we set $\alpha=\nicefrac{1}{255}$ and report the worst-case accuracy. Furthermore, we compute the adversaries for correctly-classified instances.

\textbf{Dataset:} We construct our methodology on top of the \textit{iNaturalist-H}, created by \cite{bertinetto2020making}. This dataset is a partition of the challenging iNaturalist 19 \cite{inat19}. 
It is known by how its class distribution follows a long-tail, resembling the imbalance of the real world. This dataset covers a total of 1010 leaf classes dominated by an 8-level phylogenetic tree. For fair comparison, we perform all our experiments on the validation set, as labels for the test set are kept private. 
We provide a detailed description of this dataset and useful statistics on the \textbf{Supplemental Material}.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Curriculum for Hierarchical Adversarial Training}

\begin{figure}[t]
    \centering
    \includegraphics[width=0.90\columnwidth]{images/fig curriculum.png}
    \caption{\textbf{Overview of CHAT.} Our hierarchical curriculum has two steps: the warm up (upper Figure) and the end-to-end training (bottom Figure). The warm up consist on transferring the weights and biases from the parent node to its offspring. The second step consist on training the model's parameters $\Theta$, $W^{l+1}$ and $b^{l+1}$ in a end-to-end manner.
    }
    \label{fig:curriculum}
\end{figure}

In order to defend our model against accurate and severe attacks, we propose CHAT: Curriculum for Hierarchical Adversarial Training. Inspired by human learning, we create a curriculum-based training to learn all the nodes by progressively increasing the difficulty of the task, \textit{i.e.} iteratively deepening the current level $l$ of tree to $l+1$ at each stage. Our curriculum comprises two iterative steps: the warm up and the end-to-end training. Figure \ref{fig:curriculum} illustrates a stage on our curriculum training. For the first step, consider $W^l$ and $b^l$ to be the weights and biases of the current classifier at the $l$-th stage of the curriculum. When updating the step from $l$ to $l+1$, the size of the weights of $f$ must change to account for the increase in the number of classes. Thus, we initialize a new classifier $f_{W^{l+1}, b^{l+1}}$, with $W^{l+1} \in \mathbb{R}^{n_{l+1} \times m}$ and $b^{l+1} \in \mathbb{R}^{n_{l+1}}$. Then, we provide a warm up for the weights $W^{l+1}$ and bias $b^{l+1}$ by transferring the parameters from each node $j$ to all its children. Formally, for all $i \in C_{l,l+1}(j)$ we apply:
\begin{equation}
    \begin{split}
        W_i^{l+1} &= W_j^l \\
        b_i^{l+1} &= b_j^l
    \end{split}
\end{equation}
Due to properties 2 and 3 of the transition operations in section \ref{sec:notation}, we ensure \textit{(i)} that there is always at least an offspring at each step, and \textit{(ii)} that there are no child nodes that descend from two parents. The second step consists on training all parameters of both the feature extractor, $\Theta$, and of the linear classifier, $W^{l+1}$ and $b^{l+1}$, in a end-to-end manner. The optimization process uses the labels from the current stage, namely $Y_{l+1}$, to minimize the cross-entropy loss. Furthermore, we robustify the model on this step by replacing the training with any adversarial learning method \cite{Wang_2019_ICCV, free2019, madry2017}. We iterate these stages until convergence at the leaf nodes. We enforce that the number of epochs at each stage is closely related to the number of nodes at each level. 


To train our models to be robust, we adopt an Adversarial Training~\cite{madry2017} inspired strategy. 
In particular, we follow the computationally-efficient \textit{Free Adversarial Training} (FAT) technique \cite{free2019}, which exploits each forward-backward pass to optimize both model parameters and the adversarial examples used for training. 
FAT has three hyper-parameters of interest: the number of times each adversarial example is replayed, $m$, the bound for the adversarial examples, $\epsilon$, and the size of the steps for optimization, $\alpha$.

==> sections/04_old_new_results.tex <==
 \section{Experiments}
 
%  \begin{figure*}[t]
%      \centering
%      \begin{subfigure}[b]{0.33\textwidth}
%         \includegraphics[width=\textwidth]{images/lha.png}
%         \caption{LHA Assessment}
%      \end{subfigure}
%      \hfill
%      \begin{subfigure}[b]{0.33\textwidth}
%         \includegraphics[width=\textwidth]{images/gha.png}
%         \caption{GHA Assessment}
%      \end{subfigure}
%      \hfill
%      \begin{subfigure}[b]{0.33\textwidth}
%         \includegraphics[width=\textwidth]{images/nha.png}
%         \caption{NHA Assessment}
%      \end{subfigure}
%      \caption{\textbf{Hierarchical Attack Evaluation.} We evaluate the performance of FAT on our hierarchical attacks with 50 iterations at each target height. The inclusion of our curriculum boost all metrics for all levels compared to the baseline. Acc stands for Accuracy and AM Average Mistake. (a) LHA is the strongest accuracy-related attack among the proposed ones. It even surpasses the PGD when setting the height $h$ to 5 or 6. (b) The GHA enjoys a balanced between severity and accuracy. (c) The NHA is the most severe but less successful attack among the set of hierarchical attacks.}
%      \label{fig:main_results}
%  \end{figure*}

 \begin{figure*}[t]
     \centering
     \begin{subfigure}[b]{0.33\textwidth}
        \includegraphics[width=\textwidth]{images/lha_test.pdf}
        \caption{LHA Assessment}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.33\textwidth}
        \includegraphics[width=\textwidth]{images/gha_test.pdf}
        \caption{GHA Assessment}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.33\textwidth}
        \includegraphics[width=\textwidth]{images/nha_test.pdf}
        \caption{NHA Assessment}
     \end{subfigure}
     \caption{\textbf{Hierarchical Attack Evaluation.} We evaluate the performance of FAT on our hierarchical attacks with 50 iterations at each target height on the test set. The inclusion of our curriculum boost all metrics for all levels compared to the baseline. Acc stands for Accuracy and AM Average Mistake. (a) LHA is the strongest accuracy-related attack among the proposed ones. It even surpasses the PGD when setting the height $h$ to 5 or 6. (b) The GHA enjoys a balanced between severity and accuracy. (c) The NHA is the most severe but less successful attack among the set of hierarchical attacks.}
     \label{fig:main_results}
 \end{figure*}

\input{tables/best-models}

\subsection{Curriculum-Enhanced Models against Hierarchical Attacks}


\textbf{Implementation Details.} For all our experiments we follow the experimental setup of \cite{bertinetto2020making}. We initialize a ResNet-18 \cite{resnet16} from ImageNet-pretrained \cite{imagenet_cvpr09} weights and then train the network for $200,000$ steps. We use the Adam optimizer \cite{adam2018} with $\beta_1=0.9$ and $\beta_2=0.999$, learning rate of $10^{-5}$, no weight decay, and a mini batch-size of $256$. We fix the updates in curriculum stages to occur at $2\%$, $4\%$, $6\%$, $15\%$, $25\%$ and $35\%$ of the training iterations.


\textbf{Model Selection.} We assess the effects of our new attacks against our CHAT-enhanced models. For a fair comparison between the vanilla and CHAT-enhanced models, we selected the models that provided the best robustness against PGD50 on the validation set. We explore the space of parameters $m \in \{ 2, 4, 6, 8\}$ and $\alpha\in \{\nicefrac{1}{255}, \nicefrac{2}{255}, \nicefrac{4}{255}, \nicefrac{6}{255}\}$ for the standard and hierarchy-enhanced models to search for the best-performing models for all $\epsilon \in \{\nicefrac{4}{255}, \nicefrac{6}{255}, \nicefrac{8}{255}\}$. We report each model's hyperparameters and performance on the validation set in Table \ref{tab:best-models}. The results show that the proposed CHAT enhances \textit{all} metrics on the clean and PGD50 settings by a large margin. 
We underscore that all curriculum-enhanced models were trained with a higher number of iterations $m$. 
We suspect that a higher number of iterations per height will increase even further the gap. Nonetheless, a complete study on the curriculum aspect of the training is out of the scope of this paper. Also, the step sizes of the models are large in comparison to their perturbation budget. Wang and Zhang~\cite{Wang_2019_ICCV} evidence that some models enjoy similar robustness for larger step sizes and fewer iterations when trained adversarially on the CIFAR dataset. Although we are tackling a higher-dimensional dataset, we observe this phenomenon too. FAT approximates a 1-step PGD training routine. Thus, large step sizes may further enhance adversarial robustness.

Once we choose all the best models, we quantify the effectiveness of our attacks on the testing set. Figure~\ref{fig:main_results} report the results for LHA50@$h$, GHA50@$h$ and NHA50@$h$ in the test set. These results demonstrate that introducing CHAT improves both the adversarial accuracy and severity metrics for \textit{all} models. The results of LHA present an average increase of $1.45\%$ for the robust accuracy and an average mistake decrease of $0.18$. The GHA and NHA present an average boost on the robust accuracy of $1.72\%$ and $1.91\%$, respectively. Furthermore, The average mistake metric decreases by $0.16$ for GHA and NHA. We attribute these gains to the curriculum's semantic partition, which demonstrates that semantically-coherent representation spaces enhance model robustness.


We further observe that the average mistake saturates at heights greater than or equal to 4. In contrast, the accuracy does not reach such a plateau. This event seems contradictory to the result of Figure \ref{fig:ha-ablations}. Nonetheless, the average mistake metric on this table considers both instances that initially were erroneous and not perturbed and those whose attack was successful. 


\subsection{Ablation Studies}

This section studies the effects of harnessing both our proposed CHAT and FAT to enhance the adversarial robustness and reduce the adversarial severity. We evaluate these effects by conducting standard PGD attacks to compute the accuracy and the average mistakes on regular and adversarial setups. From the side of the attacks, we first explore the effect of the number of iterations for PGD and report our results in Table \ref{tab:pgd-iterations}. From these results, we conclude that having $50$ iterations is reasonable for a clear evaluation. Thus, for all evaluations of adversarial robustness, we report numbers with respect to PGD50.

From the training side, we study two factors of interest: the curriculum and the number of iterations between curriculum stages. We train the ResNet-18 with a perturbation budget of $\epsilon=4$, a step size of $\alpha = 2$ and $m=8$ iterations to evaluate all our ablations.

\input{tables/pgd-iterations}
\input{tables/curr_ablation}

\textbf{Weight Transfer.} At each stage of the curriculum, the size of the linear classifier $f$ increases. The changing size of this layer implies that new weights are required. While these weights can be optimized by first initializing them from scratch, we propose a to start optimization from ``warm'' initialization for such weights, which we refer to as a \textit{warm-up stage}. This warm-up stage first instantiates a new classifier and then uses the weights of the old classifier to initialize the new one. Thus, here we assess the impact of employing the warm-up stage in contrast to \textit{(i)} employing no curriculum (Standard) and \textit{(ii)} a naive initialization from scratch at each curriculum stage (Scratch).

We report the results of this experiment in Table \ref{tab:curr_ablation}. Our results show that the sole inclusion of hierarchical information into FAT (``Scratch'' \textit{vs.} ``Standard'' in Table \ref{tab:curr_ablation}) greatly improves accuracy and diminishes the error severity on both clean and PGD50 settings. Moreover, employing our warm-up strategy when changing between hierarchical levels boosts performance metrics further (``CHAT (Ours)'' \textit{vs.} ``Scratch'' in Table \ref{tab:curr_ablation}). Since the Cross-Entropy ignores the relationship between labels, semantically dissimilar classes may be adjacent in the representation space. Although previous works \cite{bilal2018do} show that Cross-Entropy is capable of learning class hierarchies, our experiments suggest that employing a curriculum encourages semantically-similar classes to lie closer in representation space. We argue that this may be because they have a disjoint hyperspace for coarse classes as a prior, learned previously in the curriculum stages.

\textbf{Step Spacing.} The number of iterations used during parameter optimization can have large consequences on final performance. Since a curriculum on a hierarchy implies a changing number of classes at each curriculum stage, the amount of optimization iterations run at each stage becomes an influential factor on performance. Thus, we assess the effect of the amount of iterations to optimize each curriculum stage. 

In particular, we test two spacing strategies between curriculum stages: a naive linear spacing and our proposal, an exponential-like spacing. The linear spacing runs each curriculum for an equal number of iterations (the total number of iterations divided by the number of curriculum stages). On the other hand, our approach considers that the number of nodes at a given tree level increases exponentially. Thus, our approach assigns optimization iterations as an exponential function in the curriculum stage.

We report our results on Table \ref{tab:curr_spacing}. These results suggest that providing an exponentially-increasing number of iterations for optimizing the classes at each height of the tree leads to higher-performing \textit{and} more robust models. Combining these results with the evidence from Table \ref{tab:curr_ablation}, we argue that the evidence presented here implies that inducing hierarchy-aware priors is key to training more accurate and robust models. Using a linear spacing, we enforce this phenomenon: the small difference on Average Mistake values shows a well semantically disjoint space for the parent nodes. Nonetheless, the amount iterations available on the last stage does not enable the convergence into a local minimum for the leaf nodes.

\begin{table}[t]
    \centering
    \begin{tabular}{c||cc|cc} \toprule
        \multirow{2}{*}{\textbf{Curriculum}} & \multicolumn{2}{c|}{Clean} & \multicolumn{2}{c}{PGD50} \\
                       & \textbf{Acc}  & \textbf{AM}   & \textbf{Acc}   & \textbf{AM}\\ \midrule
        Linear        & 26.39          & 2.97          & 10.52          & 3.04\\
        Ours          & 34.11          & 2.98          & 12.15          & 3.01\\ \midrule
        Change        & \textbf{+7.72} & \textit{+0.01}& \textbf{+1.63} & \textbf{-0.03} \\\bottomrule
    \end{tabular}
    \vspace{2mm}
    \caption{\textbf{Effect of the Curriculum Steps.} We test two different curriculums and report both accuracy (Acc) and Average Mistake (AM) for clean and PGD50 adversaries. We test an exponential-like curriculum, labelled as ours, and a linear one. Given the exponential growth of the number of nodes at each level of the hierarchy tree, an exponential-like curriculum fits perfectly. \textbf{Bold} changes show gains and in \textit{italic} losses.}
    \label{tab:curr_spacing}
\end{table}

\begin{figure}[th]
    \centering
    \includegraphics[width=\columnwidth]{images/ha-ablations.png}
    \caption{\textbf{Hierarchical Attack effects.} We plot the Difference between Clean and Robust Accuracy (``Accuracy Drop'') against the flipped Average Mistake. The LHA generates semantically similar variances to each instance, while GHA creates dissimilar noise. The NHA creates weak but severe attacks as the curve is below the other ones. The number on top of each point of the curve represents the height of the hierarchical attack.}
    \label{fig:ha-ablations}
\end{figure}

\textbf{Hierarchical Attacks.} Recall that our proposed hierarchy-aware attacks have different objectives in mind, all related to inducing mistakes of varying severities. In order to visualize each effect, we plot on Figure~\ref{fig:ha-ablations} the trade-off between \textit{(i)} the Accuracy Drop (``Clean Accuracy'' minus ``Robust Accuracy'') against \textit{(ii)} the average mistake of those instances whose the attack was successful (``Flipped Average Mistake''). The former dimension looks at how powerful an attack is, and the latter reviews the severity of the successful attack. Thus, the ideal attack should be at the most upper-right corner of the plot.

The results show the intended effects of each attack: The LHA and GHA produce inverse effects, the former being semantically similar and stronger attacks, and the latter more severe but less effective attacks. Note that GHA@1 is equal to standard PGD. We expected the standard PGD to outperform all other attacks in the accuracy metric because it has a broader range of information. To our surprise, both LHA@6 and LHA@5 achieve slightly larger accuracy drops (small margins of $0.09$ and $0.05$ points, respectively). We attribute this result to the existence of useless or uninformative gradients that hinder the effectiveness of gradient-based attacks, as observed by previous studies \cite{pmlr-v80-athalye18a, papernot2017}.

The most severe attack, in terms of semantic mistakes, is our newly proposed NHA. This attack aims at generating adversaries that induce large semantic mistakes; on average, we find average mistakes of at least 0.86 and up to 1.67 points compared to the standard PGD50. Note that NHA generates noise to change the general appearances of the instance (the semantic distance between the original and target classes is significant). In contrast, the other attacks target specific classes, therefore presumably adding class-specific variations. Also, the LHA and GHA attacks are not as effective at degrading accuracy compared to the standard PGD. Since some images may contain semantic regions similar to some classes, the PGD attack already covers this spectrum of ranges. In contrast, our proposed attacks have a reduced sight of these classes.

==> sections/04old_results.tex <==
\section{Experiments}
%We first introduce the hierarchical dataset, the evaluation protocol and necessary details to replicate our results. Then, we perform a rigorous ablation study on our proposed components. Finally, we present our main results to assess the robustness and severity of error induced by our novel attacks. 

 \begin{figure*}[t]
     \centering
     \begin{subfigure}[b]{0.33\textwidth}
        \includegraphics[width=\textwidth]{images/lha.png}
        \caption{LHA Assessment}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.33\textwidth}
        \includegraphics[width=\textwidth]{images/gha.png}
        \caption{GHA Assessment}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.33\textwidth}
        \includegraphics[width=\textwidth]{images/nha.png}
        \caption{NHA Assessment}
     \end{subfigure}
     \caption{\textbf{Hierarchical Attack Evaluation.} We evaluate the performance of FAT on our hierarchical attacks with 50 iterations on each level. The inclusion of our curriculum boost all metrics for all levels compared to the baseline. Acc stands for Accuracy and AM Average Mistake. (a) LHA is the strongest accuracy-related attack among the proposed ones. It even surpasses the PGD when setting the level $l$ to 5 or 6. (b) The GHA enjoys a balanced between severity and accuracy. (c) The NHA is the most severe but less successful attack among the set of hierarchical attacks.}
     \label{fig:main_results}
 \end{figure*}

\input{tables/best-models}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%




\subsection{Curriculum-Enhanced Models against Hierarchical Attacks}


\textbf{Implementation Details.} For all our experiments we follow the experimental setup of \cite{bertinetto2020making}. We initialize a ResNet-18 \cite{resnet16} from ImageNet-pretrained \cite{imagenet_cvpr09} weights and then train the network for $200,000$ steps. We use the Adam optimizer \cite{adam2018} with $\beta_1=0.9$ and $\beta_2=0.999$, learning rate of $10^{-5}$, no weight decay, and a mini batch-size of $256$. We fix the updates in curriculum stages to occur at $2\%$, $4\%$, $6\%$, $15\%$, $25\%$ and $35\%$ of the training iterations.


\textbf{Model Selection.} We assess the effects of our new attacks against our CHAT-enhanced models. For fair comparison between the vanilla and CHAT-enhanced models, we selected the models that provided the best robustness against PGD50. 
We explore the space of parameters $m \in \{ 2, 4, 6, 8\}$ and $\alpha\in \{\nicefrac{1}{255}, \nicefrac{2}{255}, \nicefrac{4}{255}, \nicefrac{6}{255}\}$ for the standard and hierarchy-enhanced models to search for the best-performing models for all $\epsilon \in \{\nicefrac{4}{255}, \nicefrac{6}{255}, \nicefrac{8}{255}\}$. 
We report each model's hyperparameters and performance in Table \ref{tab:best-models}. The results show that the proposed CHAT enhances \textit{all} metrics on the clean and PGD50 settings by a large margin. We underscore that all curriculum-enhanced models were trained with a higher number of iterations $m$. We suspect that a higher number of iterations per level will increase even further the gap. Nonetheless, a full study on the curriculum aspect of the training is out of the scope of this paper. Also, the step sizes of the models are high in comparison of their perturbation budget. Wang and Zhang~\cite{Wang_2019_ICCV} evidence that some models enjoy similar robustness for larger step sizes and fewer iterations when trained adversarially on the CIFAR dataset. Although we are tackling a higher-dimensional dataset, we observe this phenomenon too. FAT can be considered as an approximation of 1-step PGD training. Thus, large step sizes may further enhance adversarial robustness.

%\textbf{Benchmark Evaluation.} 
Once all the best models are chosen, we quantify the effectiveness of our attacks. Figure~\ref{fig:main_results} report the results for LHA50@$h$, GHA50@$h$ and NHA50@$h$. These results demonstrate that introducing CHAT improves both the adversarial accuracy and severity metrics for \textit{all} models. The results of LHA present an average increase of $1.54\%$ for the robust accuracy and an average mistake decrease of $0.19$. The GHA and NHA present an average boost on the robust accuracy of $1.84\%$ and $1.95\%$, respectively. Furthermore, The average mistake metric decreases by $0.16$ for GHA and NHA. We attribute these gains to the semantic partition generated by the curriculum, which serves as a demonstration that semantically-coherent representation spaces enhance model robustness.


We further observe that the average mistake saturates at levels greater than or equal to 4. In contrast, the accuracy does not reach such a plateau. This event seems contradictory to the result of Figure \ref{fig:ha-ablations}. 
%Nonetheless, the average mistake metric on these tables only considers instances that initially were erroneous and not perturbed. 
Nonetheless, the average mistake metric on this table considers both instances that initially were erroneous and not perturbed and those whose the attack was successful. 
Therefore, the actual severity is much higher. The average decrease on this perturbed metric is $0.22$, $0.12$ and $0.09$ for the LHA, GHA and NHA, respectively. We provide further experimental results with the adversarial average mistake in the \textbf{Supplementary Material}.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Ablation Studies}

In this section we study the effects of harnessing both our proposed CHAT and FAT to enhance the adversarial robustness and reduce the adversarial severity. We evaluate these effects by conducting standard PGD attacks to compute the accuracy and the average mistakes on both regular and adversarial setups. From the side of the attacks, we first explore the effect of the number of iterations for PGD, and report our results in Table \ref{tab:pgd-iterations}. From these results we conclude that having $50$ iterations is reasonable for a clear evaluation. Thus, for all evaluations of adversarial robustness we report numbers with respect to PGD50.

From the side of training, we study two factors of interest: the curriculum and the amount of iterations between curriculum stages. We train the ResNet-18 with a perturbation budget of $\epsilon=4$, a step size of $\alpha = 2$ and $m=8$ iterations to evaluate all our ablations.

\input{tables/pgd-iterations}
\input{tables/curr_ablation}

\textbf{Weight Transfer.} At each stage of the curriculum, the size of the linear classifier $f$ increases, \textit{i.e.} the number of weights changes as more classes appear when considering lower levels of the hierarchy. The changing size of this layer implies that new weights are required. While these weights can be optimized by first initializing them from scratch, we propose  a to start optimization from ``warm'' initialization for such weights, which we refer to as a \textit{warm-up stage}. This warm-up stage first instantiates a new classifier and then uses the weights of the old classifier to initialize the new one. Thus, here we assess the impact of employing the warm-up stage in contrast to \textit{(i)} employing no curriculum (Standard) and \textit{(ii)} a naive initialization from scratch at each curriculum stage (Scratch).

We report the results of this experiment in Table \ref{tab:curr_ablation}. Our results show that the sole inclusion of hierarchical information into FAT (``Scratch'' \textit{vs.} ``Standard'' in Table \ref{tab:curr_ablation}) greatly improves accuracy and diminishes the error severity on both clean and PGD50 settings. Moreover, employing our warm-up strategy when changing between hierarchical levels boosts performance metrics further (``CHAT (Ours)'' \textit{vs.} ``Scratch'' in Table \ref{tab:curr_ablation}). Due to the fact that the Cross-Entropy ignores the relationship between labels, semantically dissimilar classes may be adjacent in the representation space. Although previous works \cite{bilal2018do} show that Cross-Entropy is capable of learning class hierarchies, our experiments suggest that employing a curriculum encourages semantically-similar classes to lie closer in representation space. We argue that this may be because they have a disjoint hyperspace for coarse classes as a prior that is learnt in previous curriculum stages.

\textbf{Step Spacing.} The number of iterations used during parameter optimization can have large consequences on final performance. Since a curriculum on a hierarchy implies a changing number of classes at each curriculum stage, the amount of optimization iterations run at each stage becomes a consequential factor on performance. Thus, we assess the effect of the amount of iterations for which each curriculum stage is optimized. 

In particular, we test two spacing strategies between curriculum stages: a naive linear spacing and our proposal, an exponential-like spacing. The linear spacing runs each curriculum for an equal number of iterations (the total number of iterations divided the number of curriculum stages). Our approach, on the other hand, considers how the number of nodes at a given level of a tree increases exponentially with the depth of the tree. Thus, our approach assigns optimization iterations as a function that is exponential in the curriculum stage which is being optimized.

We report our results on Table \ref{tab:curr_spacing}. These results suggest that providing an exponentially-increasing number of iterations for optimizing each level of the tree leads to higher-performing \textit{and} more robust models. Combining these results with the evidence from Table \ref{tab:curr_ablation}, we argue that evidence presented here implies that inducing hierarchy-aware priors is key to training more accurate and robust models. By using a linear spacing we enforce this phenomena: the small difference on Average Mistake values shows a well semantically disjoint space for the parent nodes. Nonetheless, the amount iterations available on the last stage does not enable the convergence into a local minimum for the leaf nodes. %\juan{not sure about the last two sentences.}


\begin{table}[t]
    \centering
    \begin{tabular}{c||cc|cc} \toprule
        \multirow{2}{*}{\textbf{Curriculum}} & \multicolumn{2}{c|}{Clean} & \multicolumn{2}{c}{PGD50} \\
                       & \textbf{Acc}  & \textbf{AM}   & \textbf{Acc}   & \textbf{AM}\\ \midrule
        Linear        & 26.39          & 2.97          & 10.52          & 3.04\\
        Ours          & 34.11          & 2.98          & 12.15          & 3.01\\ \midrule
        Change        & \textbf{+7.72} & \textit{+0.01}& \textbf{+1.63} & \textbf{-0.03} \\\bottomrule
    \end{tabular}
    \vspace{2mm}
    \caption{\textbf{Effect of the Curriculum Steps.} We test two different curriculums and report both accuracy (Acc) and Average Mistake (AM) for clean and PGD50 adversaries. We test an exponential-like curriculum, labelled as ours, and a linear one. Given the exponential growth of the number of nodes at each level of the hierarchy tree, an exponential-like curriculum fits perfectly. \textbf{Bold} changes show gains and in \textit{italic} losses.}
    \label{tab:curr_spacing}
\end{table}

\begin{figure}[th]
    \centering
    \includegraphics[width=\columnwidth]{images/ha-ablations.png}
    \caption{\textbf{Hierarchical Attack effects.} We plot the Difference between Clean and Robust Accuracy (``Accuracy Drop'') against the flipped Average Mistake. The LHA generates semantically similar variances to each instance while GHA create dissimilar noise. The NHA creates weak but severe attacks as the curve is below the other ones. The number on top of each point of the curve represents the level of the hierarchy in which the attack was conducted.}
    \label{fig:ha-ablations}
\end{figure}



\textbf{Hierarchical Attacks.} Recall that our proposed hierarchy-aware attacks are created with different objectives in mind, all related to inducing mistakes of varying severities. In order to visualize each effect, we plot on Figure~\ref{fig:ha-ablations} the trade off between \textit{(i)} the Accuracy Drop (``Clean Accuracy'' minus ``Robust Accuracy'') against \textit{(ii)} the average mistake of those instances whose the attack was successful (``Flipped Average Mistake''). The former dimension looks at the how powerful is an attack. The latter reviews the severity of the successful attack. Thus, the ideal attack should be at the most upper-right corner of the plot.

The results show the intended effects of each attack: The LHA and GHA produce inverse effects, the former being semantically similar and stronger attacks and the latter more severe but less effective attacks. Note that GHA@1 is equal to standard PGD. We expected the standard PGD to outperform all other attacks in the accuracy metric because it has a wider range of information. To our surprise, both LHA@6 and LHA@5 are capable of achieving slightly larger drops in accuracy (small margins of $0.09$ and $0.05$ points, respectively). We attribute this result to the existence of useless or uninformative gradients that hinder the effectiveness of gradient-based attacks, as observed by previous studies \cite{pmlr-v80-athalye18a, papernot2017}. %\juan{I'm not sure how to introduce this figure. I think it needs a bit more explanation.}

The most severe attack, in terms of semantic mistakes, is our newly proposed NHA. This attack aims at generating adversaries that induce large semantic mistakes; on average we find average mistakes of at least 0.86 and up to 1.67 points compared to the standard PGD50. Note that NHA generates noise in order to change general appearances of the instance (the semantic distance between the original and target classes is large), while the other attacks target specific classes, therefore presumably adding class-specific variations. Also, the LHA and GHA attacks are not as effective at degrading accuracy, compared to the standard PGD. Since some images may contain semantic regions similar to some classes, the PGD attack already covers this spectrum of ranges. In contrast, our proposed attacks have a reduced sight of these classes.





==> tables/gha.tex <==
\begin{table*}[t]
    \centering
    \begin{tabular}{c|c||cc|cc|cc|cc|cc|cc} \toprule
        \multirow{2}{*}{$\epsilon$} & \multirow{2}{*}{C} & \multicolumn{2}{c|}{GHA50 @1} & \multicolumn{2}{c|}{GHA50 @2} & \multicolumn{2}{c|}{GHA50 @3} & \multicolumn{2}{c|}{GHA50 @4} & \multicolumn{2}{c|}{GHA50 @5} & \multicolumn{2}{c}{GHA50 @6} \\
                      && Acc   & AM    & Acc   & AM    & Acc   & AM    & Acc   & AM    & Acc   & AM    & Acc   & AM    \\ \midrule
        4 &            & 12.33 &  3.20 & 14.71 & 3.32  & 15.07 & 3.33  & 15.56 &  3.34 & 17.52 &  3.34 & 18.42 & 3.33  \\
        4 & \checkmark & 13.36 &  3.05 & 15.97 & 3.18  & 16.47 & 3.19  & 17.01 &  3.20 & 19.33 &  3.21 & 20.39 & 3.19  \\ \midrule
        6 &            & 7.13  & 3.44  & 8.55  & 3.54  & 8.82  & 3.55  & 9.14  & 3.56  & 10.69 & 3.58  & 11.60 & 3.58  \\
        6 & \checkmark & 8.34  & 3.29  & 10.20 & 3.40  & 10.55 & 3.41  & 10.89 & 3.43  & 12.75 & 3.44  & 13.79 & 3.44  \\ \midrule
        8 &            & 4.31  & 3.71  & 5.21  & 3.79  & 5.35  & 3.79  & 5.53  & 3.80  & 6.60  & 3.82  & 7.32  & 3.82  \\
        8 & \checkmark & 6.05  & 3.49  & 7.28  & 3.58  & 7.50  & 3.58  & 7.81  & 3.60  & 9.26  & 3.62  & 10.10 & 3.62  \\ \bottomrule
    \end{tabular}
    \vspace{2mm}
    \caption{\textbf{Greater Hierarchical Attack Assessment.} We evaluate the performance of FAT on our hierarchical attacks with 50 iterations on each level. The inclusion of our curriculum boost all metrics for all levels compared to the baseline. Acc stands for Accuracy and AM Average Mistake. The GHA enjoys a balanced between severity and accuracy.}
    \label{tab:gha50}
\end{table*}


==> tables/lha.tex <==
\begin{table*}[t]
    \centering
    \begin{tabular}{c|c||cc|cc|cc|cc|cc|cc} \toprule
        \multirow{2}{*}{$\epsilon$} & \multirow{2}{*}{C} & \multicolumn{2}{c|}{LHA50 @1} & \multicolumn{2}{c|}{LHA50 @2} & \multicolumn{2}{c|}{LHA50 @3} & \multicolumn{2}{c|}{LHA50 @4} & \multicolumn{2}{c|}{LHA50 @5} & \multicolumn{2}{c}{LHA50 @6} \\
                      && Acc   & AM    & Acc   & AM    & Acc   & AM    & Acc   & AM    & Acc   & AM    & Acc   & AM    \\ \midrule
        4 &            & 14.64 &  2.98 & 14.39 & 2.99  & 13.80 & 3.02  & 12.39 & 3.12  & 12.23 & 3.15  & 12.25 &  3.17 \\
        4 & \checkmark & 16.32 &  2.81 & 16.01 & 2.82  & 15.36 & 2.86  & 13.60 & 2.97  & 13.36 &  3.01 & 13.33 &  3.02 \\ \midrule
        6 &            & 8.99  & 3.23  & 8.78  & 3.23  & 8.33  & 3.27  & 7.29  & 3.36  & 7.09  & 3.39  & 7.08  & 3.41  \\
        6 & \checkmark & 10.71 & 3.06  & 10.49 & 3.07  & 9.92  & 3.10  & 8.53  & 3.20  & 8.36  & 3.24  & 8.32  & 3.26  \\ \midrule
        8 &            & 5.54  & 3.53  & 5.45  & 3.54  & 5.13  & 3.57  & 4.31  & 3.64  & 4.24  & 3.67  & 4.27  & 3.69  \\
        8 & \checkmark & 7.65  & 3.27  & 7.52  & 3.28  & 7.05  & 3.32  & 6.11  & 3.41  & 5.92  & 3.45  & 5.98  & 3.46  \\ \bottomrule
    \end{tabular}
    \vspace{2mm}
    \caption{\textbf{Lower Hierarchical Attack Assessment.} We evaluate the performance of FAT on our hierarchical attacks with 50 iterations on each level. The inclusion of our curriculum boost all metrics for all levels compared to the baseline. Acc stands for Accuracy and AM Average Mistake. This attack is the strongest among the LHA, GHA and NHA, even the PGD when setting the level $l$ to 5 or 6.}
    \label{tab:lha50}
\end{table*}

==> tables/nha.tex <==

\begin{table*}[t]
    \centering
    \begin{tabular}{c|c||cc|cc|cc|cc|cc|cc} \toprule
        \multirow{2}{*}{$\epsilon$} & \multirow{2}{*}{C} & \multicolumn{2}{c|}{NHA50 @1} & \multicolumn{2}{c|}{NHA50 @2} & \multicolumn{2}{c|}{NHA50 @3} & \multicolumn{2}{c|}{NHA50 @4} & \multicolumn{2}{c|}{NHA50 @5} & \multicolumn{2}{c}{NHA50 @6} \\
                      && Acc   & AM    & Acc   & AM    & Acc   & AM    & Acc   & AM    & Acc   & AM    & Acc   & AM    \\ \midrule
        4 &            & 15.12 & 3.38  & 15.59 & 3.39  & 16.39 &  3.41 & 20.56 & 3.39  & 22.54 &  3.39 & 23.12 &  3.36 \\
        4 & \checkmark & 16.28 & 3.23  & 16.87 & 3.25  & 17.58 &  3.27 & 22.03 & 3.27  & 23.92 & 3.24  & 24.46 & 3.22  \\ \midrule
        6 &            & 8.63  & 3.59  & 8.88  & 3.60  & 9.29  & 3.62  & 12.85 & 3.66  & 14.71 & 3.65  & 15.24 & 3.63  \\
        6 & \checkmark & 10.29 & 3.45  & 10.54 & 3.47  & 11.09 & 3.49  & 15.20 & 3.52  & 16.96 & 3.51  & 17.49 & 3.49  \\ \midrule
        8 &            & 5.27  & 3.84  & 5.39  & 3.85  & 5.65  & 3.87  & 8.06  & 3.92  & 9.93  & 3.91  & 10.27 & 3.90  \\
        8 & \checkmark & 7.21  & 3.63  & 7.49  & 3.64  & 7.84  & 3.66  & 11.00 & 3.71  & 12.92 & 3.70  & 13.46 &  3.69 \\ \bottomrule
    \end{tabular}
    \vspace{2mm}
    \caption{\textbf{Node-based Hierarchical Attack Assessment.} We evaluate the performance of FAT on our hierarchical attacks with 50 iterations on each level. The inclusion of our curriculum boost all metrics for all levels compared to the baseline. Acc stands for Accuracy and AM Average Mistake. The NHA is the most severe but less successful attack among the set of hierarchical attacks.}
    \label{tab:nha50}
\end{table*}
